From WiscKey to Bourbon: A Learned Index for Log-Structured Merge Trees

We introduce BOURBON, a log-structured merge (LSM) tree that utilizes machine learning to provide fast lookups. We base the design and implementation of BOURBON on empirically-grounded principles that we derive through careful analysis of LSM design. BOURBON employs greedy piecewise linear regression to learn key distributions, enabling fast lookup with minimal computation, and applies a cost-benefit strategy to decide when learning will be worthwhile. Through a series of experiments on both synthetic and real-world datasets, we show that BOURBON improves lookup performance by 1.23x-1.78x as compared to state-of-the-art production LSMs.

==> Makefile <==
MAIN      = main
SRCS      = *.tex 
TARG      = $(MAIN).pdf


all: $(TARG)

pdf: $(SRCS) $(MAIN).bbl
	source ./SourceMe ; \
	pdflatex $(MAIN)
	source ./SourceMe ; \
	pdflatex $(MAIN)
	#cp main.pdf ~/Dropbox/Documents/

$(TARG): $(SRCS) $(MAIN).bbl
	source ./SourceMe ; \
	pdflatex $(MAIN)
	source ./SourceMe ; \
	pdflatex $(MAIN)
	touch $(TARG)
	#cp main.pdf ~/Dropbox/Documents/

bib: $(MAIN).bbl bib.tex

$(MAIN).bbl: $(MAIN).aux
	source ./SourceMe ; \
	bibtex -min-crossrefs=100 $(MAIN)
	# The below line is commented because usenix started checking
	# formatting for references also -- running redo-bib would 
	# squish the references without space to which the format 
	# checker would complain! 
	#./redo-bib.csh $(MAIN)

$(MAIN).aux: $(MAIN).tex
	source ./SourceMe ; \
	pdflatex $(MAIN)

clean:
	rm -f $(TARG) *.aux *~ $(MAIN).log $(MAIN).blg $(MAIN).out $(MAIN).dep

.SECONDARY: $(DVI)

==> fig-level-cdf.tex <==
\begin{figure}[t!]
\centering
\includegraphics[scale=0.9]{figs/level-cdf.pdf}
\mycaption{fig-level-cdf}{Level Lifetimes: Distribution of Time Between Changes}{The figure shows the distribution of time between changes for four levels.}
\end{figure}

==> fig-lifetime-sst-avg-rand.tex <==
\begin{figure}[t!]
\centering
\includegraphics[scale=0.78]{figs/lifetime-sst-avg-rand.pdf}
\mycaption{fig-lifetime-sst-avg-rand}{SSTable Lifetimes}{The figure shows the average lifetime of sstable files in levels $L_4$ to $L_0$.}
\end{figure}

==> fig-micro-datasets.tex <==
\begin{figure*}[t!] 
\centering
\captionsetup[subfigure]{labelformat=empty, justification=centering}

\subfloat[(a) Sequential load]
{
\begin{minipage}{0.28\textwidth}\
 \centering
\includegraphics[scale=0.43]{figs/datasets-sequential-eps-converted-to.pdf}
\end{minipage}%
}
\subfloat[(b) Random load]
{
\begin{minipage}{0.26\textwidth}\
 \centering
\includegraphics[scale=0.43]{figs/datasets-random.pdf}
\end{minipage}%
}
\subfloat[(c) Number of segments and negative internal lookups in \sysnamesmall]
{
\begin{minipage}{0.44\textwidth}\
 \centering
\input{tbl-micro}
\end{minipage}% 
}

%\hspace{-0.1in}{\footnotesize(a)(i) Synchronous Replication - Redis}\hspace{0.45in}{\footnotesize(a)(ii) Synchronous Replication - ZooKeeper}\hspace{0.45in}{\footnotesize(b) Asynchronous Replication - Redis}

%\hspace{0.5in}{\footnotesize(a) ZooKeeper}\hspace{1.3in}{\footnotesize(b) Redis (Synchronous Replication)}\hspace{0.45in}{\footnotesize(c) Redis (Asynchronous Replication)}

\vspace{-0.03in}
\mycaption{fig-micro-datasets}{Datasets and Load Orders}{(a) compares the average lookup latencies of \sysnamesmall, \sysnamesmall-level, and WiscKey for different datasets when the data is sequentially loaded; (b) shows the same when the data is randomly loaded; the numbers on the top show the improvements of \sysnamesmall\ over WiscKey. Table (c) shows the number of segments (for sequential loading) and negative internal lookups (for random loading) for different datasets in \sysnamesmall.}

\end{figure*}

==> impl.tex <==
\section{Implementation}
\label{sec-impl}


==> tbl-micro.tex <==
\setlength{\tempa}{\tabcolsep}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength{\tabcolsep}{1.1pt}

{\footnotesize
\begin{tabular} {M{1cm}|M{1.2cm}|M{1.4cm}|M{1.4cm}|M{1.4cm}}
\multirow{2}{1.5cm}{Dataset} & \multicolumn{2}{c|}{Sequential} &  \multicolumn{2}{c}{Random} \\\cline{2-5}
									 & \#segments & Average latency($\mu$s) & \#negative lookups& Average latency($\mu$s)\\\hline
									 %Sequential	NumSegments(File)	time	Gain-File		LLSM-File	
Linear	 &	900 &	2.7 &  49.2M &	5.6 \\
Seg1\%	 & 640K	&	3.1 &  29.8M &	4.9 \\
Normal	 & 705K	&	3.3	&  19M &	4.4 \\
Seg10\%	 & 6.4M	&	3.6 &  23.7M &	4.9 \\
\end{tabular}  
}

%\mycaption{tbl-micro}{Number of Segments and Negative lookups in \sysname-file}{\footnotesize The table shows the number of segments (for sequential loading) and negative lookups (for random loading) for different dataset in \sysname-file.}

\setlength{\tabcolsep}{\tempa}
